Study of horizontal flows in solar active regions based on high-resolution image reconstruction techniques

This thesis can be framed in a more general concept designated as "High resolution in solar physics". The first part of the thesis is dedicated to the topic of high-resolution observations and image restoration. It begins with a theoretical reviewing of the problem that represents the atmospheric turbulence and the instrumental aberrations on the image quality. This problem force us to implement post-facto image restoration techniques that, added to the real-time corrections performed by the Adaptive Optics, gives us images closer to reality. To have good solar observations overcoming the negative influence of the Earth' s atmosphere, one effort is being made with the development of the Sunrise mission. This project consists in a balloon-borne mission that will launch a 1-m telescope to the stratosphere and will record data with unprecedented temporal, spatial and spectral resolution. The main aim of Sunrise is to study the formation of magnetic structures in the solar atmosphere and their interaction with the convective plasma flows. The on-board instrument Imaging Magnetograph eXperiment (IMaX) will be able to produce magnetic field maps of extensive solar regions by measuring the light polarization in certain spectral lines. As a member of the IMaX team, I have developed an in-flight calibration method to characterize the aberrations affecting the images in IMaX. The second part of the thesis is centered on the study of horizontal flows in solar active regions. Data from ground-based and space observations are used as well as reconstruction techniques to restore the images. We focus on the proper motions of structures in and around solar active regions. The way to quantify the horizontal flows in the field-of-view consist of using local correlation tracking techniques that generate flow maps.

==> acknow.tex <==
% You can write this section in whichever language you like.
\prefacesection{Agradecimientos}
%\prefacesection{Acknowledgments}

Puedes escribir aqu\' \i \, tus agradecimientos o expresar tu reconocimiento
a las personas o instituciones que te han ayudado a completar tu trabajo.
\vspace{1.2cm}
%
% And your signature
%
{\flushleft{Your name here}}


==> biblio.tex <==
%
% This is the bibliography
%
\begin{thebibliography}{}
\addcontentsline{toc}{chapter}{Bibliography}
%
% Use the bibitem command to produce Chicago-style citations (see the
% chicago.sty file for details)
%

\bibitem[Beckers \& Schr\"oter(1969)]{beckers1969} 
Beckers, J. M., \& Schr\"oter, E. H. 1969, Solar Physics, 4, 303.

\bibitem[Berger et al.(1998)]{berger1998} 
Berger, T.E., L\"ofdahl, M.G., Shine, R.S.,\& Title, A.M. 1998, ApJ, 495, 923.

\bibitem[Bello(2001)]{bello2001}
Bello, C.D. Ph.D Thesis, Instituto de Astrof\'isica de Canarias, Tenerife (Spain).

\bibitem[Bellot et al.(2003)]{bellot2003}
Bellot Rubio, L.R., Balthasar, H., Collados, M., \& Schlichenmaier, R. 2003, A\&A, 403, L47.

\bibitem[Biermann(1941)]{biermann1941}
Biermann, L. 1941, Vierteljahresschr. Astron. Ges. 76, 194.

\bibitem[Bonet(1999)]{bonet1999}
Bonet, J.A., 1999, in \emph{Motions in the solar atmosphere}. A. Hanslmeier, M.Messerotti, ASLS, Vol 239. 

\bibitem[Bonet, Sobotka \& V\'azquez(1995)]{bonet1995} 
Bonet, J.A., Sobotka, M.  \& V\'azquez, M. 1995,  A\&A, 296, 241.

\bibitem[Bonet et al.(2004)]{bonet2004}
Bonet, J.A., M\'arquez, I., Muller, R., Sobotka, M., Tritschler, A.  2004,  A\&A, 423, 737.

\bibitem[Bonet et al.(2005)]{bonet2005} 
Bonet, J.A., M\'arquez, I., Muller, R., Sobotka, M., Roudier, Th.  2005, A\&A, 430, 1089.

\bibitem[Boreman(2001)]{boreman2001}
Boreman, G. D. 2001. \emph{Modulation Transfer Function in Optical and Electro-Optical Systems}, SPIE, International Society for Optical Engineering, TA1520.B67 2001.

\bibitem[Born \& Wolf (1999)]{bornwolf} 
Born, M., \& Wolf, E. \emph{Principles of Optics}, 1999, Cambridge University Press; 7 edition. 

\bibitem[Bovelet \& Wiehr(2003)]{bovelet2003} 
Bovelet, B., \& Wiehr, E.  2003, A\&A 412, 249. 

\bibitem[Brault \&White(1971)]{brault1971} 
Brault, J. W., \& White, O. R. 1971,  A\&A, 296, 241.

\bibitem[Brickhouse \& Labonte(1988)]{brickhouse1988} 
Brickhouse, N.S., \& Labonte, B.J. 1988, Sol. Phys, 115, 43.

\bibitem[Cabrera Solana et al.(2006)]{cabrera2006} 
Cabrera Solana, D., Bellot Rubio, L.R., Beck, C., Del Toro Iniesta, J.C.  2006, ApJ 649, L41. 

\bibitem[Carrington(1859)]{carrington1859} 
Carrington, R. C. 1859, MNRAS, 19, 81.

\bibitem[Casanovas(1997)]{casanovas1997} 
Casanovas, J., \emph{$1^{ st}$ Advances in Solar Physics Euroconference. Advances in the Physics of Sunspots. ASP Conference Series}, Vol. 118. 1997, p3-22.

\bibitem[Collados(1986)]{collados1986}
Collados, M. 1986, Ph.D Thesis University of La Laguna.

\bibitem[Cowling(1957)]{cowling1957} 
Cowling, T. G. 1957, Magnetohydrodynamics (New York: Wiley).

\bibitem[De Pontieu et al.(2007)]{depontieu2007} 
De Pontieu, B., Hansteen, V.H., Rouppe van der Voort, L., van Noort, M., Carlsson, M.  2007, ApJ 655, 624-641. 

\bibitem[De Rosa, Duvall \& Toomre(2000a)]{derosa2000} 
De Rosa, M., Duvall, T. L., Toomre, J.   2000a, Solar Physics, 192, 351.

\bibitem[Deng et al.(2007)]{deng2007}
Deng, N., Choudhary, D.P., Tritschler, A., Denker, C., Liu, C., \& Wang, H.  2007, ApJ 671, 1013-1021.

\bibitem[Deng et al.(2006)]{deng2006}
Deng, N., Xu, Y., Yang, G., Cao, W., Liu, C., Rimmele, T.R., Wang, H. \& Denker, C.  2006, ApJ 644, 1278.

\bibitem[Dere, Schmieder  \& Alissandrakis(1990)]{dere1990}
Dere, K. P., Schmieder, B., \& Alissandrakis, C. E. 1990, A\&A, 233, 207.

\bibitem[Dialetis, Mein \& Alissandrakis(1985)]{dialetis1985}
Dialetis, D., Mein, P., \& Alissandrakis, C. E. 1985, A\&A, 147, 92.

\bibitem[Domingo, Fleck \& Poland(1995)]{domingo1995}
Domingo, V., Fleck, B., \& Poland, A. I. 1995, Solar Physics, 162, 1.

\bibitem[Evershed(1909)]{evershed1909}
Evershed, J. 1909, MNRAS, 69, 454.

\bibitem[Fabricius(MDCXI)]{fabriciusMDCXI}
Fabricius, J.  \emph{De Maculis in Sole observatis ...,} Wittenbergae, MDCXI.

\bibitem[Gizon et al.(2000)]{gizon2000}
Gizon, L., Duvall, T.L., Jr., \& Larsen, R.M. 2000, J. Astrophys. Astron., 21, 339.

\bibitem[Gonsalves \& Childlaw(1979)]{gonsalves1979} 
Gonsalves, R. A., \& Childlaw, R. 1979, \emph{in Applications of Digital Image Processing III}, A.G. Techer (ed.), Proc. Soc. Photo-Opt. Instrum. Eng. 207, 32.

\bibitem[Gonsalves(1982)]{gonsalves1982} 
Gonsalves, R. A., 1982, Opt. Eng. 21, 829.

\bibitem[Hagenaar \& Shine(2005)]{hagenaar2005} 
Hagenaar, H.J., \& Shine, R.A. 2005, ApJ 635, 659. 

\bibitem[Hale(1908)]{hale1908} 
Hale, G.E. 1908, ApJ, 28, 315.

\bibitem[Harvey \& Harvey(1973)]{harvey1973} 
Harvey, K., \& Harvey, J. 1973, Solar Phys. 28, 61.

\bibitem[Haugen(1969)]{haugen1969} 
Haugen, E. 1969, Solar Physics, 9, 88.

\bibitem[Hirzberger et al.(1999)]{hirzberger1999} 
Hirzberger, J., Bonet, J.A., V\'azquez, M. \& Hanslmeier, A. 1999, ApJ 515, 441-454.

\bibitem[Ishikawa et al.(2007)]{ishikawa2007} 
Ishikawa, R., Tsuneta, S., kitakoshi, Y., Katsukawa, Y., Bonet, J.A., Vargas Dom\'inguez, S., Rouppe van der Voort, L.H.M., Sakamoto, Y., Ebisukaki, T. 2007, A\&A 472, 911 - 918.

\bibitem[Keil(1999)]{keil1999}
Keil, S. L., Balasubramaniam, K. S., Smaldone, L. A., \&  Reger, B. 1999, ApJ, 510, 422.

\bibitem[Keppler(1955)]{keppler1955}
Keppler, J., \emph{Gesammelte Werke}, Max Caspar, vol. XVII, M\"unchen, 1955.

\bibitem[Kosugi et al.(2007)]{kosugi2007}
Kosugi, T., Matsuzaki, K., Sakao, T., et al. 2007, Sol. Phys., 243, 3.

\bibitem[Kubo et al.(2007)]{kubo2007}
Kubo, M., Shimizu, T., \& Tsuneta, S. 2007, ApJ 659, 812.

\bibitem[L\"ofdahl(1996)]{lofdahl1996} 
L\"ofdahl, M.G. 1996, Ph.D Thesis  Stockholm University. 

\bibitem[L\"ofdahl \& Scharmer(1994)]{lofdahl1994} 
L\"ofdahl, M.G., Scharmer, G.B. 1994, A\&A Suppl. Ser. 107, 243.

\bibitem[L\"ofdahl(2002)]{lofdahl02MFBD} 
L\"ofdahl, M.G. 2002, Proc. SPIE., 4792, p.146.

\bibitem[Maltby(1975)]{maltby1975}
Maltby, P. 1975, Solar Physics, 43, 91.

\bibitem[M\'arquez, S\'anchez-Almeida \& Bonet(2006)]{marquez2006}
M\'arquez, I., S\'anchez-Almeida, J., \& Bonet, J.A. 2006, ApJ 638, 553.

\bibitem[Mart\'inez Pillet et al.(1994)]{pillet1994}
Mart\'inez Pillet, V., Lites, B. W., Skumanich, A., Degenhardt, D. 1994, ApJ, 425, 113.

\bibitem[Meyer et al.(1974)]{meyer1974}
Meyer, F., Schmidt, H.U., Weiss. N. O., \& Wilson, P.R. 1974, Proc. IAU Symp., 56, p.235.

\bibitem[Molowny-Horas(1994)]{molownyphd1994} 
Molowny-Horas, R. 1994, Ph.D Thesis University of Oslo.

\bibitem[Molowny-Horas \& Yi(1994)]{molowny1994} 
 Molowny-Horas, R., \& Yi, Z. 1994, ITA (Oslo) Internal Rep. No. 31.

\bibitem[Moore(1981)]{moore1981} 
Moore, R. L., 1981, ApJ 249, 390.

\bibitem[Muller(1976)]{muller1976} 
Muller, R. 1976, Solar Physics, 48, 101.

\bibitem[Noll(1976)]{noll1976}
Noll, R. J., 1976. J. Opt. Soc. Am. 66(3), 207.

\bibitem[November(1986)]{november1986}
November, L.J. 1986, Appl. Opt., 25, 392.

\bibitem[November \& Simon(1988)]{november1988}
November, L.J., \& Simon, G.W. 1988, ApJ 333, 427.

%\bibitem[Nye et al.(1988)]{nye1988}
%Nye, A., Bruning, D., Labonte, B. J. 1988, Solar Phys. 115, 251.
\bibitem[Parker(1979)]{parker1979}
Parker, E. N. 1979, ApJ, 230, 905.

\bibitem[Paxman et al.(1992)]{paxman1992} 
Paxman, R.G., Schulz, T.J., Fienup, J.R. 1992, J.Opt.Soc.Am. A9, 7, 1072.

\bibitem[Ravindra(2006)]{ravindra2006}
Ravindra, B. 2006, Solar Phys. 236, 297.

\bibitem[Rimmele(1995)]{rimmele1995}
Rimmele, T. R. 1995, ApJ, 445, 511.

\bibitem[Rimmele(2000)]{rimmele2000}
Rimmele, T.R. 2000, 'Solar adaptive optics'. In: P.L. Wizinowich (ed.): \emph{Adaptive Optical System Technologies}, Vol. 4007 of Proc. SPIE. pp. 218-231.

\bibitem[Roudier, Bonet \& Sobotka(2002)]{roudier2002} 
Roudier, Th., Bonet, J.A., \& Sobotka, M. 2002, A\&A, 395, 249	.	
		
\bibitem[Roudier et al.(2003)]{roudier2003} 
Roudier, Th., Ligni\`eres, F., Rieutord, M., Brandt, P.N., \& Malherbe, J.M. 2003, A\&A, 409, 299.	

\bibitem[Roudier \& Muller(2004)]{roudier2004} 
Roudier, Th., \& Muller, R. 2004, A\&A, 419, 757.

\bibitem[Sainz Dalda \& Mart\'inez Pillet(2005)]{sainz2005}
Sainz Dalda, A., Mart\'inez Pillet, V. 2005, ApJ, 662, 1176.

\bibitem[Scharmer et al.(2000)]{scharmer2000}
Scharmer, G.B., Shand, M., L\"ofdahl, M. G., Dettori, P. M., \& Wei, W.  2000, 'A Workstation Based Solar/Stellar Adaptive Optics System'. In: P.L. Wizinowich (ed.): \emph{Adaptive Optical System Technologies}, Vol. 4007 of Proc. SPIE. pp. 239-250.

\bibitem[Scharmer et al.(2003a)]{scharmer2003a}
Scharmer G. B., Bjelksj\"o K., Korhonen, T.K., Lindberg, B. \& Petterson, B. 2003a, Proc. SPIE. 4853, 341.

\bibitem[Scharmer et al.(2003b)]{SSTAO}
Scharmer G. B., Dettori, P. M., L\"ofdahl, M. G. \& Shand, M. 2003b, Proc. SPIE, 4853, 370.

\bibitem[Scheiner(1623-30)]{scheiner1623-30}
Scheiner, C. 1626-30, \emph{Rosa Ursina}, Bracciano.

\bibitem[Schlichenmaier \& Schmidt(2000)]{schlichenmaier2000}
Schlichenmaier, R., \& Schmid, W. 2000, A\&A, 337, 897.

\bibitem[Schmidt(1991)]{schmidt1991}
Schmidt, M. 1991, Geophys. Astrophys. Fluid Dynamics, 62, 249.

\bibitem[Schrijver \& Zwann(2000)]{schrijver2000} 
Schrijver, C. J., \& Zwann, C. 2000, Solar and stellar magnetic activity. Cambridge U Press.

\bibitem[Sheeley(1969)]{sheeley1969} 
Sheeley, N.R. 1969, Solar Phys. 9, 347.

\bibitem[Sheeley \& Bhatnagar(1971)]{sheeley1971} 
Sheeley, N.R. \& Bhatnagar, A. 1971, Solar Phys. 19, 338.

\bibitem[Sheeley(1972)]{sheeley1972} 
Sheeley, N.R. 1972, Solar Phys. 25, 98.

\bibitem[Shine, Simon \&  Hurlburt(2000)]{shine2000} 
Shine, R. A., Simon, G. W., \& Hurlburt, N. E. 2000, Solar Physics. 193, 313.

\bibitem[Sch\"ussler et al(2002)]{schussler2002} 
Sch\"ussler, M. 2002, Astronomische Nachrichten, vol. 323, no. 3/4, p. 377-382.

\bibitem[Sch\"ussler et al(2003)]{schussler2003} 
Sch\"ussler, M., Shelyag, S., Berdyugina, S., V\"ogler, A., \& Solanki, S.K. 2003, ApJ, 597, L173.

\bibitem[Sobotka et al.(1999)]{sobotka1999}
Sobotka, M., Vazquez, M., Bonet, J.A., Hanslmeier, A., \& Hirzbeger, J. 1999, ApJ, 511, 436.

\bibitem[Sobotka \& S\"utterlin(2001)]{sobotka2001}
Sobotka, M.,  \& S\"utterlin, P. 2001, A\&A, 380, 714.

\bibitem[Sobotka \& Roudier(2007)]{sobotka2007}
Sobotka, M., \& Roudier, T. 2007, A\&A, 472, 277.

\bibitem[Stanchfield, Thomas \& Lites(1997)]{stanchfield1997}
Stanchfield, D.C.H., Thomas, J. H.,  \& Lites, B. W. 1997, ApJ, 477, 485.

\bibitem[Thomas \& Weiss(1992)]{thomas1992}
Thomas, J. H.,  \& Weiss, N. O. 1992, in Sunspots: Theory and Observations, Thomas, J. H., Weiss, N.O (eds.), Kluwer Academic Publishers, 3.

\bibitem[Thomas et al(2002)]{thomas2002}
Thomas, J. H., Weiss, N. O., Tobias, S. M. \& Brummell, N. H. 2002, Nature 420, 390-393.

\bibitem[Title et al(1986)]{title1986}
Title, A. M., Frank, Z. A., Shine, R. A., Tarbell, T. D.,, Topka, K. P., Scharmer, G.,  \& Schmidt, W. 1993, ApJ,403, 780.

\bibitem[Title et al(1993)]{title1993}
Title, A. M., Tarbell, T., Simon, G., and the SOUP team. 1986, Adv. Space Res., 6, 253.

\bibitem[Vargas Dom\'inguez et al.(2007)]{vargas2007}
Vargas Dom\'inguez, S., Bonet, J.A., Mart\'inez Pillet, V., Katsukawa, Y., Kitakoshi, Y., Rouppe van der Voort, L. 2007, ApJL, 660, L165.

\bibitem[Vargas Dom\'inguez et al.(2008)]{vargas2008}
Vargas Dom\'inguez, S., Rouppe van der Voort, L., Bonet, J.A., Mart\'inez Pillet, V., van Noort, M., Katsukawa, Y. 2008, ApJ, 679,900.

\bibitem[Van Noort, Rouppe van der Voort \& L\"ofdahl(2005)]{momfbd2005}
Van Noort. M., Rouppe van der Voort, L., L\"ofdahl, M. G. 2005, Sol. Phys., 228, 191.

\bibitem[V\"ogler et al.(2005)]{vogler2005}
V\"ogler, A., Shelyag, S., Sch\"ussler, M., Cattaneo, F., Emonet, T., \& Linde, T. 2005, A\&A, 429, 335.

\bibitem[Vrabec(1974)]{vrabec1974}
Vrabec, D. 1974, Proc. IAC Symp., 56, p.201.

\bibitem[Westendorp Plaza et al.(1997)]{westendorp1997}
Westendorp Plaza, C., del Toro Iniesta, J.C., Ruiz Cobo, B., Mart\'inez Pillet, V., Lites, B.W., Skumanich, A. 1997, Nature, 289, 47.

\bibitem[Wilson(1973)]{wilson1973} 
Wilson, P. R. 1973, Solar Physics, 32, 435.

\bibitem[Yi(1992)]{yi1992} 
Yi, Z. 1992, Ph.D Thesis University of Oslo.

\bibitem[Yurchyshyn et al(2001)]{yur2001} 
Yurchyshyn, V. B., Wang, H., \& Goode, P. R. 2001, A\&A, 550, 470.

\bibitem[Zernike(1934)]{zernike1934} 
Zernike, F. 1934. Physica 1, 689.

\bibitem[Zirin \& Wang(1989)]{zirin1989} 
Zirin, H., Wang, H. 1989, Solar Phys. 119, 245.

\bibitem[Zwaan(1992)]{zwaan1992} 
Zwaan, C. 1992, Proceedings of the NATO Advanced Research Workshop on the Theory of Sunspots, Cambridge, United Kingdom, p. 75-100.


\vspace{10mm}

\hspace{5mm}{ \LARGE IMaX documentation}\\

\noindent
IMaX Final Optical Design, SUN-IMaX-RP-IX200-023\\
IMaX Technical Note, SUN-IMaX-TN-IX200-022\\

\vspace{7mm}
\noindent
\hspace{5mm}{ \LARGE Websites}\\

\noindent
\emph{http://www.iac.es/galeria/svargas/movies.html} \\
\emph{http://www.iac.es/galeria/svargas/corks.html}\\
\emph{http://www.iac.es/proyect/IMaX/}\\
\emph{http://www.solarphysics.kva.se}\\
\emph{http://www.solarphysics.kva.se/LaPalma}\\
\emph{http://solar-b.nao.ac.jp/hsc\_e/darts\_e.shtml}\\
\emph{http://www.csiro.au}\\	

		






\end{thebibliography}

